MultiModalQA: Complex Question Answering over Text, Tables and Images

When answering complex questions, people can seamlessly combine information from visual, textual and tabular sources. While interest in models that reason over multiple pieces of evidence has surged in recent years, there has been relatively little work on question answering models that reason across multiple modalities. In this paper, we present MultiModalQA(MMQA): a challenging question answering dataset that requires joint reasoning over text, tables and images. We create MMQA using a new framework for generating complex multi-modal questions at scale, harvesting tables from Wikipedia, and attaching images and text paragraphs using entities that appear in each table. We then define a formal language that allows us to take questions that can be answered from a single modality, and combine them to generate cross-modal questions. Last, crowdsourcing workers take these automatically-generated questions and rephrase them into more fluent language. We create 29,918 questions through this procedure, and empirically demonstrate the necessity of a multi-modal multi-hop approach to solve our task: our multi-hop model, ImplicitDecomp, achieves an average F1of 51.7 over cross-modal questions, substantially outperforming a strong baseline that achieves 38.2 F1, but still lags significantly behind human performance, which is at 90.1 F1

==> related_work.tex <==
\section{Related Work}

\at{\begin{enumerate}[topsep=0pt,itemsep=0ex,parsep=0ex]
    \item Paragraph1, Mainly discuss HybridQA and ManyModalQA as closely related work. (this could be in the intro as well)
    \item Paragraph2, Can we find past Multi Modality datasets? not necessarily in QA. 
    \item Paragraph3, Discuss Multi-Hop complex questions answering works such as WikiHop, HotpotQA, The web as a KB etc ...
    \item Paragraph4, Discuss "cavities" and multi-hop analysis work such as Sewon Mins, Mohit Bansal etc...
    \item -------- Submission to Supp line ------------
    \item Paragraph4, Can we find references for image list questions?
\end{enumerate}}




